Physics of Strongly Magnetized Neutron Stars

There has recently been growing evidence for the existence of neutron stars possessing magnetic fields with strengths that exceed the quantum critical field strength of $4.4 \times 10^{13}$ G, at which the cyclotron energy equals the electron rest mass. Such evidence has been provided by new discoveries of radio pulsars having very high spin-down rates and by observations of bursting gamma-ray sources termed magnetars. This article will discuss the exotic physics of this high-field regime, where a new array of processes becomes possible and even dominant, and where familiar processes acquire unusual properties. We review the physical processes that are important in neutron star interiors and magnetospheres, including the behavior of free particles, atoms, molecules, plasma and condensed matter in strong magnetic fields, photon propagation in magnetized plasmas, free-particle radiative processes, the physics of neutron star interiors, and field evolution and decay mechanisms. Application of such processes in astrophysical source models, including rotation-powered pulsars, soft gamma-ray repeaters, anomalous X-ray pulsars and accreting X-ray pulsars will also be discussed. Throughout this review, we will highlight the observational signatures of high magnetic field processes, as well as the theoretical issues that remain to be understood.

==> abs <==
Physics of Strongly Magnetized Neutron Stars

Alice K. Harding (GSFC) and Dong Lai (Cornell)

93 pages. Reports on Progress in Physics, in press (2006)

There has recently been growing evidence for the existence of neutron
stars possessing magnetic fields with strengths that exceed the
quantum critical field strength of $4.4 \times 10^{13}$ G, at which
the cyclotron energy equals the electron rest mass.  Such evidence has
been provided by new discoveries of radio pulsars having very high
spin-down rates and by observations of bursting gamma-ray sources
termed magnetars.  This article will discuss the exotic physics of
this high-field regime, where a new array of processes becomes
possible and even dominant, and where familiar processes acquire
unusual properties.  We review the physical processes that are
important in neutron star interiors and magnetospheres, including the
behavior of free particles, atoms, molecules, plasma and condensed
matter in strong magnetic fields, photon propagation in magnetized
plasmas, free-particle radiative processes, the physics of neutron
star interiors, and field evolution and decay mechanisms.  Application
of such processes in astrophysical source models, including
rotation-powered pulsars, soft gamma-ray repeaters, anomalous X-ray
pulsars and accreting X-ray pulsars will also be discussed.
Throughout this review, we will highlight the observational signatures
of high magnetic field processes, as well as the theoretical issues
that remain to be understood.
